Focused Large Language Models are Stable Many-Shot Learners

In-Context Learning (ICL) enables large language models (LLMs) to achieve rapid task adaptation by learning from demonstrations. With the increase in available context length of LLMs, recent experiments have shown that the performance of ICL does not necessarily scale well in many-shot (demonstration) settings. We theoretically and experimentally confirm that the reason lies in more demonstrations dispersing the model attention from the query, hindering its understanding of key content. Inspired by how humans learn from examples, we propose a training-free method FocusICL, which conducts triviality filtering to avoid attention being diverted by unimportant contents at token-level and operates hierarchical attention to further ensure sufficient attention towards current query at demonstration-level. We also design an efficient hyperparameter searching strategy for FocusICL based on model perplexity of demonstrations. Comprehensive experiments validate that FocusICL achieves an average performance improvement of 5.2% over vanilla ICL and scales well with many-shot demonstrations.

==> rebuttal.tex <==
R1 4-3.5-4

Paper Summary:
This paper studies in-context learning (ICL) for large language models (LLMs). It discusses the reason, i.e. distraction, why using more in-context demonstrations does not nessacerily lead to performance gain in ICL. Then it proposes FocusICL, to allocate attention to demonstrations in a hierarchical manner. Experiments show that FocusICL results in stable ICL performance with many ICL desmonstrations.

Summary Of Strengths:
The paper is well-motivated, well-written, and easy to follow.

The studied problem is critical and provides novel understanding of ICL.

It proposes a novel approch to increase the ICL performance, which stablizes ICL performances in many-shot setting.

Summary Of Weaknesses:

We sincerely appreciate your thorough review and the constructive suggestions you have provided. We have carefully read them and engaged in thoughtful discussions (detailed below). We believe this will further contribute to enhancing the quality of our manuscript.

> I wonder if the authors have tried FocusICL with chain-of-thought together. Or, does FocusICL help LLMs focus more on the reasoning paths when used together with CoT?

- Yes, our results on GSM8K demonstrate that using FocusICL alongside CoT is effective. As shown in Tables 1, 2, and 3, FocusICL significantly enhances LLMs' ability of chain-of-thought reasoning compared to ICL on GSM8K. We further computed the average attention weights on reasoning paths for LONGCHAT-7B-V1.5-32K on GSM8K. The results demonstrate that FocusICL achieves an average attention weight of 0.0042 on tokens within reasoning paths, which is higher than the 0.0032 under ICL. This indicates that the improvement in model performance stems from its increased focus on addressing the current problem.

# 是的，我们在GSM8K上的结果是FocusICL配合CoT一起使用的。如Table1、2、3所示，相比于ICL，FocusICL显著提升了LLM利用chain-of-thought推理的性能。我们进一步统计了LONGCHAT-7B-V1.5-32K在GSM8K上对于reasoning paths的平均注意力权重，结果显示FocusICL对于reasoning path中token的平均注意力权重为0.0042，高于ICL下的0.0032，这明确了性能的提升是模型更专注于解决当前problem带来的。

> What would happen if we drop a few demonstrations with minimal attention? E.g. given 10 demonstrations, FucosICL finds 3 of them are limitedly attended to. What's the performance if we drop these 3 and use the rest 7 for plain ICL?

- We implemented your valuable suggestion as follows: on the GSM8K dataset, using LONGCHAT-7B-V1.5-32K, we first identified the 10 demonstrations with the lowest average attention weights out of 96, discarded them, and then applied ICL to the remaining 86 demonstrations. The results below show that filtering demonstrations based on attention effectively enhances the performance of ICL, validating our motivation for filtering based on attention. However, this method requires re-encoding demonstrations and performs less effectively than the finer-grained token-level filtering method (TRIVIALITY) used by FocusICL.
|Method|Accuracy|
|:--:|:--:|
|ICL|9.93|
|ICL-drop last 10|10.79|
|TRIVIALITY|11.00|
|FocusICL|12.28|

# 我们尝试了您所提出的建议，具体设置为在GSM8K数据集上，我们用LONGCHAT-7B-V1.5-32K先找到96条demonstrations中平均注意力权重最小的10条并舍弃，然后在剩下的86条中应用ICL。我们发现通过attention可以对demonstration进行有效的筛选，从而提升ICL的性能，这佐证了我们依据attention进行过滤的动机。不过该方法需要对demonstrations重复编码，同时性能低于FocusICL所采用的更细粒度的从token-level进行过滤的方法。
|Method|Accuracy|
|:--:|:--:|
|ICL|9.93|
|ICL-drop last 10|10.79|
|TRIVIALITY|11.00|
|FocusICL|12.28|

> It is not clear whether the order of demonstrations affect the attention calculated by FocusICL and the performance of FocusICL. Elaborating on that will be hlepful for readers to better understand FocusICL.

- Our main experiments in Table 1, 2 and 3 reported the average results of FocusICL over 5 randomly selected sets of demonstrations, reflecting its robustness. We further explored the impact of varying the order of demonstrations within a set five times on FocusICL's attention and performance. The table below illustrates the results of LONGCHAT-7B-V1.5-32K model applying FocusICL on the GSM8K dataset. It's evident that FocusICL is generally robust to changes in the order of demonstrations.
|Order|Accuracy|
|:--:|:--:|
|1st order|12.20|
|2nd order|12.16|
|3rd order|12.44|
|4th order|12.31|
|5th order|12.25|

# 我们的主实验所报告的结果是FocusICL在5次随机选择demonstrations下得到结果的平均值，反映了结果的鲁棒性。我们进一步尝试了在一组demonstrations内5次改变它们的顺序对FocusICL的attention和performance的影响情况。下表展示了在GSM8K数据集上LONGCHAT-7B-V1.5-32K模型应用FocusICL的结果。可以看到基本上FocusICL对于demonstrations顺序的改变是足够鲁棒的。
| Order     |  Accuracy |
| :--: | :--:|
| 1st order | 12.20|
| 2nd order  | 12.16 |
| 3rd order     |   12.44 ｜
| 4th order | 12.31 |
| 5th order      |    12.25 |



R2 2.5-2.5-3

Paper Summary:
This paper, through theoretical analysis and experiments, confirms that the dispersion of model attention from the query leads to a performance decline as the number of demonstrations increases in many-shot in-context learning. To address this issue, the authors propose masking the attention weights of less important demonstrations and introducing a hierarchical attention method. Experiments conducted on five datasets and three models demonstrate the effectiveness of the proposed method compared to baseline approaches.

Summary Of Strengths:
The authors provide a clear theoretical analysis demonstrating how an increase in the number of demonstrations causes the model's attention to become dispersed from the query, and they support this with experimental evidence.
The author compares their method with baseline approaches across various models, showcasing its superiority.
The author analyzes the efficiency gains achieved through the hierarchical attention method.

Summary Of Weaknesses:

> The experimental scenario presumes the model has access to a large number of in-distribution demonstrations for queries, which may be impractical in real-world situations. Examining the model’s performance in out-of-distribution scenarios could yield more valuable insights.

- We conducted the following experiments to investigate your interesting suggestion: We used the training sets of the PIQA and ARCE datasets as candidate sets for demonstrations and tested the LLM's performance on PIQA when applying ICL and FocusICL, as shown in the table below. We found that when using out-of-domain demonstrations, both ICL and FocusICL's performance decreases. Specifically, FocusICL shows a slightly more performance decline, although its performance still outperforms ICL. We hypothesize that this is because when there is limited useful knowledge in the demonstrations, FocusICL's effectiveness in extracting beneficial knowledge through hierarchical attention strategies is diminished.
|Source of Demos|Method|Accuracy|
| :--: | :--:|:--:|
|PIQA|ICL|57.42|
|PIQA|FocusICL|60.83|
|ARCE|ICL|57.12|
|ARCE|FocusICL|59.82|

# 实验CSQA的demonstration下对于PIQA的提升
1. ARCE demonstrations + PIQA sample + ICL
2. ARCE demonstrations + PIQA sample + FocusICL
|Source of Demos|Method|Accuracy|
| :--: | :--:|:--:|
|PIQA|ICL|57.42|
|PIQA|FocusICL|60.83|
|ARCE|ICL|57.12|
|ARCE|FocusICL|59.82|

58128

> When comparing with baseline methods, the author only considered the maximum number of demonstrations. Evaluating the performance of methods with varying numbers of demonstrations, as shown in Figure 5, might offer more meaningful insights.

- In Figure 5, we compared the performance trends of FocusICL with ICL (which we consider the most important and widely used baseline) as the number of demonstrations increases. We observed that FocusICL consistently outperforms ICL across various settings. Recognizing the potential for additional insights from comparisons with other baselines, we also evaluated LONGCHAT-7B-V1.5-32K on the CSQA dataset to assess performance changes with varying numbers of demonstrations across different methods, as shown in the table below. We have the following findings:

1. **EarilyStop**: It achieved optimal performance at demonstration number 32 and truncated subsequent demonstrations.

2. **StructICL**: Initially, its computation and performance were same to ICL. Later, structuring the input led to performance improvement.

3. **Triviality**: By filtering out irrelevant content, it mitigated the impact of attention dispersion, increasing the optimal demonstration number from 32 to 64.

4. **FocusICL**: It consistently achieved performance gains from a larger number of demonstrations.

| Demonstration Number|8|16|32|64|128|
|:-:|:-:|:-:|:-:|:-:|:-:|
|ICL|45.91|46.98|47.89|46.60|47.58
|EarilyStop|45.91|46.98|47.89|47.89|47.89|
|StructICL|45.91|46.98|47.89|49.18|50.25|
|Triviality|46.31|47.94|49.26|49.28|48.97|
|FocusICL|46.31|47.94|49.26|50.03|50.70|



# 我们在Figure 5 中对比了FocusICL与ICL（我们认为是最重要和广泛使用的基线）随着demonstration数量增长的性能变化情况，并发现FocusICL在各种settings下都展现了更好的性能。我们认可与其他基线也进行类似的比较可能带来更多insights，因此我们在CSQA数据集上比较了LONGCHAT-7B-V1.5-32K在各种methods下性能随demonstration数量变化的表现，如下表所示。我们有以下发现：1.EarilyStop在最佳表现点，也即demonstration number=32时对后续的demonstration进行了截断。2. StructICL在前期和ICL运算过程、性能相同，后期通过将输入结构化使性能得到了提升。3. Triviality通过过滤无用的内容减轻了注意力分散的影响，将最佳demonstration数量从32提升到了64. 4. FocusICL实现了从更多的demonstration中获得持续的性能增益。
| Demonstration Number|8|16|32|64|128|
|:-:|:-:|:-:|:-:|:-:|:-:|
|ICL|45.91|46.98|47.89|46.60|47.58
|EarilyStop|45.91|46.98|47.89|47.89|47.89|
|StructICL|45.91|46.98|47.89|49.18|50.25|
|Triviality|46.31|47.94|49.26|49.28|48.97|
|FocusICL|46.31|47.94|49.26|50.03|50.70|

> The observation in Sec 5.5 regarding "More demonstrations are needed when they have a closer relationship" is questionable. This might simply be due to the CountA dataset significantly deviating from the model's pre-trained knowledge.

- We agree with your point of view, and we will modify the statement "More demonstrations are needed when they have a closer relationship" to "More demonstrations are needed when the task is complex for the model," thereby integrating both perspectives.

# 我们认同您的说法，并将会把表述"More demonstrations are needed when they have a closer relationship"更改为“More demonstrations are needed when the task对于模型来说是复杂的”，从而融合两种观点。

> Reporting the actual values of inference time and memory cost for the method proposed, in comparison to the baseline methods, would be meaningful.

- We agree with your viewpoint, and it would be beneficial to report more detailed efficiency quantification results. We present the efficiency of our method and baseline in the following table, including throughput and GPU memory utilization.

| Methods|queries/min|Max Memory (GB)|
|:-:|:-:|:-:|
|ICL|1.54|～40|
|EarlyStop|1.82|～36|
|StructICL|1.95｜～40|
|Triviality|1.52|～40|
|FocusICL|1.97|～40|


> Comments Suggestions And Typos

- We greatly appreciate your kind feedback on the typos, and we will correct these issues in the final version.

# 感谢指出typos！我们将在最终版本中修正这些问题。
There are reference errors in lines 230 and 798.
The "maximum available number of demonstrations" mentioned in line 374 is not shown in Table 7.
Confidence: 3 =  Pretty sure, but there's a chance I missed something. Although I have a good feel for this area in general, I did not carefully check the paper's details, e.g., the math or experimental design.
Soundness: 2.5
Overall Assessment: 2.5


R3 3-2.5-5

Paper Summary:
This paper claims that performance diminishes as the number of in-context exemplars increases. To address this, the authors introduce a masked attention mechanism to filter out the irrelevant, i.e., less important tokens, during the inference step.

Summary Of Strengths:
The research problem is interesting. Revisiting the attention of context is crucial to adjust the attention of the generated tokens.
Experimental results show that, compared to two baselines, the proposed solution achieved better performance.
Summary Of Weaknesses:

> Tokens with less weight contribute less to the generated tokens, so why should masking them boost performance?

-  While tokens with less weight contribute less to the generated tokens, their greater quantity can still lead to a dispersion of model attention, as shown in Figure 1. After filtering out tokens with less weight, FocusICL allocates stable and sufficient attention to the current problem, thereby improving performance, as illustrated in Figure 6.

# 尽管Tokens with less weight contribute less to the generated tokens，但是它们的数量较多，从而会导致模型注意力的分散，如图1所示。在对Tokens with less weight进行过滤后，FocusICL分配了对于当前problem稳定、足够的attentions，从而提升了效果，如图6所示。

> It is unreasonable to mask the test example itself.

- As shown in Equation 8, we only mask tokens belonging to the demonstrations and do not mask the test example itself.

# 如公式8所示，我们只mask属于demonstration的tokens，不mask the test example itself

> There is no ablation study supporting this claim. It would be better to compare performance by masking tokens above the threshold and using random masking.

- Our ablation studies compare masking low-attention tokens with not masking tokens, as seen in Table 1, 2, and 3 for the comparison between TRIVIALITY and ICL. Masking low-attention tokens consistently leads to performance improvements. We think the setting of random masking lacks practical meanings; hence, it is not included in the comparison.

# 我们的ablation study是通过比较mask低attention的tokens和不mask tokens进行的，如Table1、2、3中的TRIVIALITY和ICL之间的对比，mask低attention的tokens能带来稳定的性能提升。我们认为random masking没有现实意义，因此没有对比。

> The conducted experiments are exclusive to text classification, a task that does not benefit much from extended context [1]. It would be valuable to see how the proposed solution works on generative tasks and other classification tasks, including NLI and multiple question answering.

- We evaluated LLM's performance with FocusICL on the GSM8K benchmark for CoT reasoning, testing the effectiveness of FocusICL in generative reasoning tasks. Additionally, we assessed LLMs' capabilities on the CountA dataset, which evaluates LLMs' inference abilities and serves a similar testing purpose to NLI tasks.

# 我们在GSM8K benchmark上测试了LLM在CoT推理时FocusICL的性能，这检验了LLM在生成式推理任务上应用FocusICL的有效性。我们还测试了LLMs在CountA数据集上的能力，该数据集考验了LLM的inference能力，起到了和NLI任务类似的检验效果。

> The claim that "StructICL designs focus on extending available context length" is not true. StructICL rescales the attention values of the generated tokens, making it applicable similarly to the proposed solution. However, all figures compare the proposed solution to a vanilla model.

- From the original statement in the StructICL paper, "However, conventional in-context learning is usually restricted by length constraints, rendering it ineffective to absorb supervision from a large number of examples. In order to go beyond few shots, we introduce structured prompting," we inferred that "StructICL designs focus on extending available context length."

Additionally, we agree that StructICL is applicable in our settings. Therefore, we have compared various LLMs and benchmarks with StructICL in Table 1, 2, and 3.


# 我们从StructICL原文中的表述“However, conventional in-context learning is usually restricted by length constraints, rendering it ineffective to absorb supervision from a large number of examples. In order to go beyond few shots, we introduce structured prompting.” 总结出了"StructICL designs focus on extending available context length".
此外，我们认同StructICL is applicable in our settings，因此在Table1、2、3中的各个LLMs和数据集上都与StructICL进行了比较。

# 

Comments Suggestions And Typos:

> The proposed solution aims to enhance model stability, but the reported results lack metrics such as standard deviation or significance tests (T-test).

- We acknowledge your point. In fact, to ensure the reliability of our results, each reported result is the average of 5 runs. We will supplement relevant standard deviations or significance tests in the revised version.

# 我们认可您说的这一点，事实上为了确保结果的可靠性，我们所汇报的每个result都是5次运行下的均值。我们将在修订版本中补充相关的standard deviation or significance tests

> The paper does not link to recent work, including PCW[2], which is very relevant, and NBCE [3], a recent publication.

- Similar to StructICL, PCW and NBCE focus on achieving context extension under limited computational resources, while FocusICL addresses the issue of model attention dispersion in many-shot settings.

Specifically, PCW and NBCE achieve context window extension by avoiding attention and pooling operations between context windows, thereby preserving the uniqueness of each window. In contrast, FocusICL also avoids attention between context windows but implements hierarchical attention to reweight attention across different batches. The primary goal is to ensure the model focuses more on beneficial demonstrations.

We will cite PCW and NBCE in the revised version accordingly.


# 和StructICL类似，PCW与NBCE都关注如何在有限的计算资源下实现Context Extension，而FocusICL更关注于解决长上下文窗口时的模型注意力分散问题。
具体来说，PCW和NBCE分别通过避免context window间的attention和pooling操作保留唯一的window从而实现对于context window的扩展。对比之下FocusICL也避免context window间的attention，不同的是，FocusICL实施了Hierarchical Attention从而实现对于不同batch的attention reweight，核心目的是让模型更关注有益的demonstrations。
我们将在修订版本中对PCW和NBCE进行引用。

> The mathematical formalization is non-standard, resulting in difficulty in understanding and interpreting the equation. It is suggested to reformulate equation (2) in order to facilitate a direct comparison with equation (3). For details, refer to the reference “Why can GPT learn in-context? language models secretly perform gradient descent as meta-optimizers.” and equations (8) and (9) as well.

- We conducted more detailed formula derivations in the anonymous link (https://anonymous.4open.science/r/Detailed-Derivations-3FB7/derivation.pdf), aiming to enhance your understanding of the key aspects of our derivation process.

Furthermore, we hope to clarify that the main difference between our approach and that in [1] lies in the consolidation of similar terms. We consider the comparison between $\hat{x}(W_0,\delta W_{FT})$ and $\hat{h}_r(W_{ZSL}+\delta W_{ICL})$ to be equivalent and clear, as well as the comparison between $\hat{x}W_0 + \hat{x}\delta W_{FT}$ and $\hat{h}_r W_{ZSL}+\hat{h}_r \delta W_{ICL}$.


# [1]中的表述和我们的主要区别在于合并了同类项，我们希望搞清楚$\hat{x}(W_0,\delta W_{FT})$ 和 $\hat{h}_r(W_{ZSL}+\delta \W_{ICL})$是否比$\hat{x}W_0 + \hat{x}\delta W_{FT}$与$\hat{h}_r W_{ZSL}+\hat{h}_r \delta \W_{ICL}$之间的对比更加direct？

> In lines 401~402, “…achieving an average of 5.2\% (3.31 points) performance improvement ”，what is the relationship between “5.2\%” and “3.31 points”.

- In Tables 1, 2, and 3, across all settings, the average accuracy for ICL is \(63.87\%\), while for FocusICL it is \(67.18\%\). The difference between the two is \(3.31\%\). This \(3.31\%\) increment relative to \(63.87\%\) implies a \(5.18\%\) improvement.

在table1、2、3的所有settings上，ICL的Avg accuracy是$63.87\%$，FocusICL的Avg accuracy是$67.18\%$，二者差值是$3.31\%$，$3.31\%$的增量相比于$63.87\%$意味着$5.18\%$的提升。

> Rishabh et al. [4] found that extending the context without adjusting attention can enhance performance on complicated tasks.

- Indeed, when tasks are challenging and models struggle to comprehend with minimal demonstrations, LLMs become demonstration-hungry, aligning with our findings on CountA in Figure 5. In this scenario, we demonstrate that FocusICL, compared to ICL, better enables LLMs to benefit from a greater number of demonstrations, as illustrated by vicuna-7b-v1.5-16k and Meta-Llama-3-8B-Instruct on the CountA dataset, as shown in Figure 5.

# 是的，当任务困难、模型难以通过少量demonstration理解时，LLM将变得demonstration-hungry，这和我们在Figure 5中CountA上的结论一致。在这种情况下，我们证明，FocusICL相比于ICL能更好地帮助LLM从更多的demonstrations中受益，如Figure 5中vicuna-7b-v1.5-16k与Meta-Llama-3-8B-Instruct在CountA数据集上所展示的那样。

> Line 294 should cite PCW [2] or StructICL as it follows the same design .

- Yes, we accept your suggestion and will cite it in the revised version.

# 是的，我们接受您的建议，并将在修订版本中进行引用。



R4 2.5-2.5-3

Paper Summary:
ICL allows LLMs to quickly adapt to new tasks using a few demonstrations, but scaling to many-shot settings will not bring stable performance improvements. This paper identify that the primary cause is the dispersion of model attention due to an increasing number of demonstrations, which hinders the model's ability to focus on the query. To solve this, they propose FOCUSICL, a training-free method that uses triviality filtering to mask unimportant tokens and hierarchical attention to ensure sufficient focus on the query. Their method also includes an efficient hyperparameter search strategy based on model perplexity. Experiments show that FOCUSICL improves performance by 5.2\% over vanilla ICL and scales well with many-shot demonstrations.

Summary Of Strengths:
Innovative Approach. The introduction of FOCUSICL is a novel solution to the problem of attention dispersion in many-shot ICL settings.

Performance Improvement. The method demonstrates a significant improvement in performance (5.2\%) over traditional ICL approaches.

Summary Of Weaknesses:
> The proof is not detailed. How do you derive the Eq. 5? Could you provide more detailed proof in the appendix? What does “J” mean in Eq. 6. Could you give a detailed definition of each type and its corresponding shape in Sec. 3. I also do not know what the meaning of e\^s\_jk , j, k···in Eq. 10. The authors need to explain all Eqs more clearly.

- Due to the constraints of formatting detailed derivations in Comment, we have provided a more comprehensive derivation process in the following anonymous link: https://anonymous.4open.science/r/Detailed-Derivations-3FB7/derivation.pdf. We hope this helps clarify our formulas.

In Eq. 6, the index $j$ is intended to enumerate each term in $exp(h_r W_q Q_k^T)$.
Regarding Eq. 10, $e^{s_j^i}$，where $e$ denotes the base of the mathematical constant $e$ and $s_j^i$ refers to the attention score of the $j$-th token in the $i$-th batch. Therefore, Eq. 10 signifies the weighted sum of hidden states $\hat{h}_r^i$, where each batch is weighted based on the sum of attention scores of tokens within that batch, resulting in the final hidden state.

 
# 由于我们无法在Comment中以latex格式写具体的推导过程，我们将更详细的推导过程放在了该匿名链接中：https://anonymous.4open.science/r/Detailed-Derivations-3FB7/derivation.pdf
希望这有助于帮助您理解我们的公式。
Eq. 6中的j意在索引$exp(h_r W_q Q_k^T)$中的每一项。
关于Eq. 10中的$e^{s_j^i}$，$e$指的是the base of the mathematical constant e, $s_j^i$指的是第i个batch中的第j个token的attention score.因此公式 10指的是依据每个batch中token的attention score的和作为该batch的权重，对该batch对应得到的hidden state $\hat{h}_r^i$进行加权求和，作为最终的hidden state。

- The pipeline of the proposed method may not be clear enough. Which layers of models are the proposed method inserted? An ablation study on the effect of layers would be better.

> As described in Figure 3 (top right), line 264, and line 538, we implemented Triviality Filtering and Hierarchical Attention at each layer. Our preliminary experiments indicate that applying these operations at every layer achieves the best results.

如我们在如图3右上角、line 264以及line 538所描述的，我们在每一层实施了我们所提出的Triviality Filtering与Hierarchical Attention。我们的前期实验表明在每一层都进行该操作能够取得最好的效果。

> Computation Efficiency. The authors have discussed the computation efficiency of their methods in the experiment section. However, it is difficult to compute the overhead of the operation (e.g., index and comparison) in Eq. 8. As such, could you report the running time for your method and the original ICL in an experiment to justify the Computation Efficiency?

- We agree with your viewpoint, and it would be beneficial to report more detailed efficiency quantification results. We present the efficiency of our method and baseline in the following table, including throughput and GPU memory utilization.

| Methods|queries/min|Max Memory (GB)|
|:-:|:-:|:-:|
|ICL|1.54|～40|
|EarlyStop|1.82|～36|
|StructICL|1.95｜～40|
|Triviality|1.52|～40|
|FocusICL|1.97|～40|

如下是FocusICL和baselines的效率对比结果

| Methods|queries/min|Max Memory (GB)|
|:-:|:-:|:-:|
|ICL|1.54|～40|
|EarlyStop|1.82|～36|
|StructICL|1.95｜～40|
|Triviality|1.52|～40|
|FocusICL|1.97|～40|

> What happens when the chosen demonstration examples are high-quality? For example, the chosen demonstration example is similar to the test case. Could you discuss the performance difference between ICL+ demonstration Selection and ICL + demonstration Selection+ your method? You can just use the similarity of bert embedding between demonstration and test query as an example.

- We appreciate your valuable suggestion, and accordingly, we used BERT embeddings to retrieve the most relevant demonstrations. We then compared the experimental results using both ICL and FocusICL, as shown in the table below. Retrieving relevant demonstrations resulted in a 1.13\% improvement for ICL and a 1.53\% enhancement for FocusICL. This improvement is likely attributed to the hierarchical attention mechanism's ability to more effectively utilize demonstrations with substantial informative content.

|Method|Original Accuracy|Accuracy with Relevant Demonstrations|
| :--:|:--:|:--:|
|ICL|47.58|48.71|
|FocusICL|50.70|52.23|



| Method    | Improvement (%) |
|-----------|-----------------|
| ICL       | 1.13%           |
| FocusICL  | 1.53%           |

我们认为这是一个很好的提议，为此我们按照您的建议用BERT embedding检索了最相关的demonstrations并分别用ICL和FocusICL比较了实验结果，如下表所示。相关的demonstrations为ICL带来了1.13\%的进步，为FocusICL带来了1.53\%的提升。这可能源自于层次化的注意力机制能对带大量有增益信息的demonstrations进行更加充分的利用。

|Method|Accuracy|
| :--:|:--:|
|ICL|48.71|
|FocusICL|52.23|







R3-2

Thank you for your in-depth discussion and timely feedback. We will further elaborate to address your concerns.

> **Figure 3 indicates that tokens from the query are masked, which needs further clarification or justification.**

We apologize for any misunderstanding caused by Figure 3. We will explain it in detail for you. As stated in Figure 3, "(x,y) indicates the attention of x towards y." Therefore, considering the last 3 tokens in Figure 3 belong to the query, and none of the tokens in the last three columns are masked, this means tokens from the query are not masked.

> **The current ablation study only reports results for low-attention masking versus no masking. It would be more insightful to compare performance between masking tokens above a certain threshold and using random masking.**

We agree with your perspective and have conducted more detailed ablation studies accordingly. Using the LONGCHAT-7B-V1.5-32K dataset, we performed the following ablation studies on CountA dataset:

- No token masking
- Masking 40\% of tokens with the lowest attention
- Masking 40\% of tokens with the highest attention
- Randomly masking 40\% of tokens

The experimental results below demonstrate the following: compared to No Masking, randomly masking 40\% of tokens reduces accuracy from 79.04\% to 35.00\%. Masking 40\% of tokens with the highest attention leads the model to repeatedly output the word 'nobody', indicating a loss of problem-solving ability. Conversely, masking 40\% of tokens with the lowest attention significantly improves performance.

To further analyze the underlying reasons, we calculated the model's perplexity across different settings. We found that random masking and masking high-attention tokens significantly increase model perplexity, likely due to the loss of critical token information. In contrast, masking low-attention tokens decreases model perplexity, indicating that filtering trivial tokens based on posterior attention information helps the model perform tasks more confidently.

We will incorporate these ablation study results into the final version of our work.

|Method|Accuracy|Perplexity|
| :--:|:--:|:--:|
|No Masking|79.04|0.610|
|Mask 10\% tokens with lowest attention weights|85.68|0.572|
|Mask 10\% tokens with highest attention weights|0.00|10.921|
|Random Mask 10\% tokens|35.00|1.636|

> **The paper does not report on any generative tasks, which is a significant oversight.**

We tested the performance of various compared methods on the GSM8K dataset using the CoT decoding strategy. This task requires large language models (LLMs) to generate complete and accurate reasoning processes to obtain precise answers. Without generating high-quality reasoning path, LLMs are not likely to predict the right answer. We believe that in this scenario, FocusICL's generative capability has been put to the test. In the final version, we will include more generative tasks to make the experiments more comprehensive.

> **Referencing Eq. 2 of StructICL, it is clear that replacing ( M ) with a value greater than 1 should work effectively.**

M of Eq. 2 in StructICL (referred to as Scaling Factor in the original paper) acts as a hyperparameter controlling the attention weights between queries and demonstrations. They default this value to the number of groups. Their experimental results indicate that as M increases from 1 to twice the number of groups, model performance initially improves and then declines, reaching optimal performance at the default setting. In contrast, FocusICL adopts a hierarchical attention strategy that adaptively allocates and reinforces attention to queries without introducing hyperparameter. Additionally, the LLMs can assign appropriate weights to different batches based on the relevance of content within each batch. Our experimental results in Tables 1, 2, and 3 demonstrate that FocusICL achieves superior performance compared to the default setting of StructICL.

> **While I believe any masking approach could potentially improve performance, the assumption that low-attention weight tokens should be masked requires both theoretical and empirical validation.**

We agree that both theoretical and empirical validation of the masking approach would make this work more persuasive. In Section 3 of the main text, we have demonstrated through formula derivation that an increase in demonstrations and the resulting abundance of tokens can disperse the model's attention from the query, a point empirically supported by Figure 1. Building on this, our main experiment (Table 1,2,3) compares ICL with our proposed method and, as evidenced by Figure 6, proves that FocusICL can enhance performance by masking irrelevant tokens. Following your valuable suggestions, we further validated in the ablation studies mentioned above that masking important or random tokens can indeed significantly hurt the performance, which serves as a strong ablation study for our strategy. We think that we have made every effort to validate our claims on both theoretical and empirical levels.

**We would like to thank you once again for your valuable suggestions and hope that our response can alleviate your concerns. We will integrate our discussion into the final version to further enhance the quality of our paper.**

我们赞同您的观点，为此进行了更加详细的ablation studies. 在CountA数据集上，我们用LONGCHAT-7B-V1.5-32K进行了如下的ablation studies: 1. 不mask 任何token 2. mask 40\% attention最低的token 3. mask 40\% attention最高的token 4. 随机mask 40\%的tokens。实验结果如下所示：实验结果显示，相比于No Masking，随机mask 40\%的tokens会导致准确率从79.04\%下降至35.00\%，而mask 40\% attention最高的tokens则会导致模型丧失解决问题的能力（实验中模型将会重复输出单词 'nobody'）。而mask 40\% attention最低的tokens则将会带来性能的显著提升。为了进一步分析背后的原因，我们统计了各种settings下的模型perplexity，发现random masking和masking high-attention tokens 会导致模型困惑度显著上升，这可能是由于模型丧失了关键tokens的信息导致的。相比之下，masking low-attention tokens则会带来模型困惑度的降低，这说明依据attention的后验信息来过滤triviality tokens能帮助模型更有把握地完成任务。我们将把这一ablation实验结果加入到最终版本中。


|Method|Accuracy|Perplexity|
| :--:|:--:|:--:|
|No Masking|79.04|0.610|
|Mask 10\% tokens with lowest attention weights|85.68|0.572|
|Mask 10\% tokens with highest attention weights|0.00|10.921|
|Random Mask 10\% tokens|35.00|1.636|

> **The paper does not report on any generative tasks, which is a significant oversight.**

We tested the performance of various compared methods on the GSM8K dataset using the CoT decoding strategy. This task requires large language models (LLMs) to generate complete and accurate reasoning processes to obtain precise answers. Without generating high-quality reasoning path, LLMs are not likely to predict the right answer. We believe that in this scenario, FocusICL's generative capability has been put to the test. In the final version, we will include more generative tasks to make the experiments more comprehensive.

> **Referencing Eq. 2 of StructICL, it is clear that replacing ( M ) with a value greater than 1 should work effectively.**

M of Eq. 2 in StructICL (referred to as Scaling Factor in the original paper) acts as a hyperparameter controlling the attention weights between queries and demonstrations. They default this value to the number of groups. Their experimental results indicate that as M increases from 1 to twice the number of groups, model performance initially improves and then declines, reaching optimal performance at the default setting. In contrast, FocusICL adopts a hierarchical attention strategy that adaptively allocates and reinforces attention to queries without introducing hyperparameter. Additionally, the LLMs can assign appropriate weights to different batches based on the relevance of content within each batch. Our experimental results in Tables 1, 2, and 3 demonstrate that FocusICL achieves superior performance compared to the default setting of StructICL.

> **While I believe any masking approach could potentially improve performance, the assumption that low-attention weight tokens should be masked requires both theoretical and empirical validation.**

We agree that both theoretical and empirical validation of the masking approach would make this work more persuasive. In Section 3 of the main text, we have demonstrated through formula derivation that an increase in demonstrations and the resulting abundance of tokens can disperse the model's attention from the query, a point empirically supported by Figure 1. Building on this, our main experiment (Table 1,2,3) compares ICL with our proposed method and, as evidenced by Figure 6, proves that FocusICL can enhance performance by masking irrelevant tokens. Following your valuable suggestions, we further validated in the ablation studies mentioned above that masking important or random tokens can indeed significantly hurt the performance, which serves as a strong ablation study for our strategy. We think that we have made every effort to validate our claims on both theoretical and empirical levels.


我们赞同对masking approach进行both theoretical and empirical validation能使该工作更加的有说服力。在正文中的第三节，我们通过公式推导证明了更多的demonstrations带来的大量token会分散模型对于query的注意力，这一点得到了Figure 1的empiirical证明。在此基础上，我们通过主实验中ICL与我们所提出方法的对比和Figure 6证明了FocusICL能够通过mask 不重要的 tokens带来性能的提升。在您的valuable建议下，我们在上文中所提供的abalation studies进一步验证了mask重要的、随机的tokens无法带来性能的显著提升。我们认为我们已经尽了最大的努力来从both theoretical and empirical 层面验证我们的声明。

Eq. 2 of StructICL 中的M(事实上被称为Scaling Factor)作为一个超参数控制了模型对于query和demonstrations之间的注意力权重，他们将这个值默认设定为groups的数量。他们的实验结果表明，随着M从1增大到2倍的groups数量，模型性能先升后降，在默认设定处达到最优。与之相比，FocusICL采用了层次化attention策略，自适应分配、强化对于query的attention，无需引入超参数；同时模型能够为不同的batch依据batch中有益内容的多少赋予合适的权重。我们在Table 1、2、3中的实验结果表明，FocusICL相比于STRUCTICL取得了更优的性能。



